Non-volatile Tuning of Cryogenic Optical Resonators

Quantum computing, ultra-low-noise sensing, and high-energy physics experiments often rely on superconducting circuits or semiconductor qubits and devices operating at deep cryogenic temperatures (4K and below). Photonic integrated circuits and interconnects have been demonstrated for scalable communications and optical domain transduction in these systems. Due to energy and area constraints, many of these devices need enhanced light-matter interaction, provided by photonic resonators. A key challenge, however, for using these resonators is the sensitivity of resonance wavelength to process variations and thermal fluctuations. While thermo-optical tuning methods are typically employed at room temperature to mitigate this problem, the thermo-optic effect is ineffective at 4K. To address this issue, we demonstrate a non-volatile approach to tune the resonance of photonic resonators using integrated phase-change materials (PCMs) at cryogenic temperatures. In this work, we report a 10Gb/s free-carrier dispersion based resonant photonic modulator that can be tuned in a non-volatile fashion at sub-4K temperatures using a commercial silicon photonics process. This method paves the way for realizing scalable cryogenic integrated photonics with thousands of resonant devices for quantum and high-energy physics applications.

==> device_design.tex <==
\section{Modulator Device Design}
\label{sec:device_design}
Racetrack micro-ring modulator (MRM) was designed such that a section of the device could include an embedded PIN micro-heater for tuning the state of the PCM. PIN micro-heater structures can electrically reconfigure the device by inducing a micro-structural phase change from amorphous (a-GST) to crystalline (c-GST) state (called ``SET" process) and vice versa (called ``RESET" process) for GST~\cite{wuttig2017phase}. The SET process occurs when GST is maintained at a temperature above its glass transition temperature ($T_g=673 K$~\cite{zheng2020modeling}) and below the melting temperature ($T_m=888 K$~\cite{zheng2020modeling}). The RESET process occurs when GST is heated above $T_m$ and cooled down rapidly. 

\begin{figure}[h]%
\label{fig:fig1}
\centering
\includegraphics[width=0.9\textwidth]{Figures/jnl_fig1.png}
\caption{Device design: (a) Schematic illustrates the concept of tuning the MRM by inducing a phase change in the deposited PCM, (b) Device illustration of PIN micro-heater integrated with race-track MRM (c) cross-section of PIN micro-heater and mode profile simulation with 10 nm GST on waveguide}\label{fig1}
\end{figure}
